Language processing in humans and computers

Machine-learned language models have transformed everyday life: they steer us when we study, drive, manage money. They have the potential to transform our civilization. But they hallucinate. Their realities are virtual. This note provides a high-level overview of language models and outlines a low-level model of learning machines. It turns out that, after they become capable of recognizing hallucinations and dreaming safely, as humans tend to be, the language-learning machines proceed to generate broader systems of false beliefs and self-confirming theories, as humans tend to do.

==> 20-SYN/200-intro.tex <==
% !TEX root = 2-syn.tex

People speak many languages. People who speak different languages generally don't understand each other. How is it possible to have a general theory of language? 

Life is also diversified in many species, and different species generally cannot interbreed\footnote{The fact that most people do not understand each other even when they speak the same language echoes the fact that most members of the same species do not breed, but select mates through complex rituals.}. But life is a \emph{universal capability of self-reproduction}\/ and biology is a general theory of life. % General sciences of diversified phenomena are possible. 

General linguistics is based on Noam Chomsky's \emph{Cartesian assumption}\footnote{Early linguists (Humboldt, Boas, Sapir, Whorf) were mainly focused on understanding different worldviews (Weltanschauung, Weltanzicht) by understanding different languages (German, Hebrew, English, Hopi, Nahuan,\ldots).}: that all languages arise from a \emph{universal capability of speech}, innate to our species. The claim is that all of our different languages share the same \emph{deep structures}\/ embedded in our brains.% Its absence is the reason why even the animals very close to us remain unable to speak.
Since different languages assign different words to the same things, the semantic assignments of words to meanings are not a part of these universal deep structures. 
% Moreover, the assignments evolve by random mutations and appear arbitrary since, e.g., the English lexicon would remain functional if the meanings of the words ``cow'' and ``raccoon'' were swapped.\footnote{The costs of such operations can be derived from the costs of ``civilizing'' the populations of ``barbarians'' in the colonial past. Ironically, the Greek word \emph{barbarian}, denoting a speaker of a foreign language, is one of the rare examples where the meaning assignment is not entirely arbitrary since the sound does suggest the meaning.}
Chomskian general linguistics is mainly concerned with general syntax. It also studies (or it used to study) the transformations of the deep syntactic structures into the surface structures observable in particular languages, just like biology studies the ways in which the general mechanisms of heredity lead to particular organisms. Oversimplying a little, the Chomskian thesis implies that 
\begin{itemize}
\item  syntax is the main subject of modern linguistics, whereas
\item  semantics is studied in complementary ways in 
\begin{itemize}
\item philosophy of meaning, be it under the title of \emph{semiology}, or in the many avatars of \emph{structuralism}; and by different methods in 
\item search engine engineering, information retrieval indices and catalogs, user profiling, and targeted advertising. 
\end{itemize}
\end{itemize}


%
%
%
%
%
%
% A possibility of general linguistics arose from Chomsky's \emph{Cartesian assumption}\/ that, although particular languages differ on the surface, they are all based on a  \emph{universal capability of speech}. More precisely, the claim is that all of the different languages humans speak share the same \emph{deep structure}, innate to our species, transferred with our genes. --- The demarcation line between syntax and semantics is a logical consequence of this assumption. General linguistics is then split into a core theory of universal syntax, branching into its observable instantiations in particular languages, with the blurry realm of semantics on the margins. 
%
%This conundrum of a universal core branching into diverse instantiations arises not only in linguistics but in studying evolutionary processes in general. Biology studies many different species of organisms, which generally cannot interbreed, yet a general theory subsuming all of them is possible because they are all deemed to arise from a \emph{universal capability of life}.\footnote{The fact that some people do not understand each other even when they speak the same language echoes the fact that some organisms do not breed even when they are members of the same species.} 
However, the difference between the pathways from deep structures to surface structures as studied in linguistics on one hand and in biology on the other is that 
 \begin{itemize}
\item in biology, the carriers of the deep structures of life are directly observable and empirically studied in genetics, whereas 
\item in linguistics, the deep structures of syntax are not directly observable but merely postulated, as Chomsky's Cartesian foundations, and the task of finding actual carriers is left to a future science. 
\end{itemize}
This leaves the Cartesian assumption about the universal syntactic structures on a shaky ground. The emergence of large language models may be a tectonic shift of that ground. Most of our early interactions with chatbots seem to suggest that the demarcation line between syntax and semantics may not be as clear as traditionally assumed. 

To understand a paradigm shift, we need to understand the paradigm. To stand a chance to understand large language models, we need a basic understanding of the language models previously developed in linguistics. In this lecture and in the next one, we parkour through the theories of syntax and of semantics, respectively. %Skipping and jumping is always a dubious strategy, so please don't slip. But we cannot see a tectonic shift while standing on a tectonic plate. %A bird's eye view is needed. We don't interbreed with birds.



 




==> 40-LEARN/410-intro.tex <==
% !TEX root = 4-learn.tex

Anyone can drive a car. Most people even know what the engine looks like. But when you need to fix it, you need to figure out how it works.

Anyone can chat with a chatbot. Most people know that there is a Large Language Model (LLM) under the hood. There are lots and lots and lots of articles describing what an LLM looks like. Lots of colorful pictures. Complicated meshes of small components, as if both mathematical abstraction and  modular programming still need to be invented. YouTube channels with fresh scoops on LLM celebrities.  We get to know their parts, how they are connected, we know their performance, we even see how each of them changes a heat map of inputs to a heat map of outputs. One hotter than another. But do we understand how they work? Experts say that they do, but they don't seem to be able to explain it even to each other, as they continue to disagree about pretty much everything. 

\begin{figure}[!ht]
\begin{center}
\includegraphics[height=13cm]{PICS/santa-1.jpg}
\caption{Transformer architecture revealed}
\label{Fig:santa}
\end{center}
\end{figure}

Every child, of course, knows that it can be hard to explain what you just built. Our great civilization built lots of stuff that was unable to explain. Steam engines have been engineered for nearly 2000 years before scientists explained how they extract work from heat. There aren't many steam engines around anymore, but there are lots of language engines and a whole industry of scientific explanations how they work. The leading theory is that Santa Claus descended from the mountain and gave us the transformer architecture carved in a stone tablet. It changed the world, spawned offspring and competitors\ldots Just like steam engines. Which may be a good thing, since steam engines did not exterminate their creators just because the creators didn't understand them.%, or just because they could\ldots% They exploded once in a while, but the numbers of victims were comparable on both sides, and in the end, the steam engines got exterminated, and replaced. First by cars, and then by language engines. Transformers changed the world, spawned offspring and competitors.Ê.Ê. Just like steam engines. Which may not be a bad thing. Steam engines did not exterminate their creators just because they didn't understand how work is extracted from heat. But we do need to understand how LLMs extract intelligence from training.

I wasn't around in the times of steam engines, but I was around in the times of bulky computers, and when the web emerged and everything changed, and when the web giants emerged and changed the web. Throughout that time, AI research seemed like an effort towards the intelligent design of intelligence. It didn't change anything, because intelligence, like life, is an evolutionary process, not a product of intelligent design\footnote{Alan Turing explained that machine intelligence could not be achieved through intelligent designs, because intelligence itself could not be completely specified, as it is its nature to always seek and find new paths. But Turing was also the first to realize that the process of computation was not bound by designs and specifications either, but could evolve and innovate. He anticipated that machine intelligence would evolve with computation. However, three years after Turing's death, the concept of machine intelligence, which he thought and wrote about for the last 8 years of his life, got renamed to artificial intelligence, his writings sank into oblivion, and the logical systems designed to capture intelligence proliferated.}.  
%It took many decades for those logical systems to sink into oblivion, and for machine intelligence to evolve.%
Now the friendly learning machines and chatbot AIs evolved and everything is changing again. Having survived and processed the paradigm shifts of the past, I am now trying to understand the present one. Hence this course and these writings. On one hand, I probably stand no chance to say anything that hasn't been said already. Even after a lot of honest work, I remain a short-sighted non-expert. On the other hand, as far as I can tell, the gentle AI experts seem unaware of some powerful tools and ideas that evolved in the neighborhood. People clump into research communities, focus on the same things, and ignore the same things. Looking over the fence, the neighbors sometimes see what they don't see. So here is a view across the fence, with all the bad and good things that go with it.
%\begin{figure}%[!hb]
%\begin{center}
%\includegraphics[height=13cm]{PICS/steam-gpt.jpg}
%\caption{A learning machine hallucinates}
%\label{Fig:santa}
%\end{center}
%\end{figure}

%\footnote{I have been using the categorical toolkit, even when I don't mention categories, to unify fragments of math dispersed through various parts of computer science. People familiar toolkit will probably notice it in the background here.} 


